Robobarista: Object Part based Transfer of Manipulation Trajectories from Crowd-sourcing in 3D Pointclouds

There is a large variety of objects and appliances in human environments, such as stoves, coffee dispensers, juice extractors, and so on. It is challenging for a roboticist to program a robot for each of these object types and for each of their instantiations. In this work, we present a novel approach to manipulation planning based on the idea that many household objects share similarly-operated object parts. We formulate the manipulation planning as a structured prediction problem and design a deep learning model that can handle large noise in the manipulation demonstrations and learns features from three different modalities: point-clouds, language and trajectory. In order to collect a large number of manipulation demonstrations for different objects, we developed a new crowd-sourcing platform called Robobarista. We test our model on our dataset consisting of 116 objects with 249 parts along with 250 language instructions, for which there are 1225 crowd-sourced manipulation demonstrations. We further show that our robot can even manipulate objects it has never seen before.

==> features.tex <==
\section{Features for Structural SVM and Latent Structural SVM}
\label{sec:ssvm_features}
%\vspace*{\sectionReduceBot}


\subsection{Structured SVM}
For one of our baselines, we tested the structured support vector machines 
\cite{tsochantaridis2005large} using hand-coded
features and our loss function from Section~\ref{sec:metric}. We solved the SVM 
optimization
problem using the cutting plane method \cite{joachims2009cutting}.
The joint feature map used, $\phi(p, l, \tau)$, consists of a set of different factors
to capture different relations between point-cloud $p$, language $l$, and trajectory
$\tau$: $\phi(p, l, \tau) = [\phi(\tau); \phi(p, \tau); \phi(l, \tau)]$. 




\textbf{Trajectory Features} $\phi(\tau)$:
To represent trajectories of different length with small number of features,
we take an unsupervised non-linear dimensionality reduction approach.
For every trajectory $\tau$, we first compute smooth interpolated trajectory $\tau_s$
(Sec.~\ref{sec:trajrep}),
%as discussed earlier in Section~\ref{sec:trajrep},
and then normalize all trajectories $\mathcal{T}$ to same length
while preserving the sequence of gripper status.
Finally, 
a non-linear reduction method 
Isomap \cite{tenenbaum2000global}
%is applied 
is used to project to a lower dimension of 15 dimensions using 5 nearest neighbors.
%to find the non-linear mapping to lower dimension of 15 dimensions using 5 nearest neighbors.



\textbf{PointCloud-Trajectory Features} $\phi(p,\tau)$:
To capture overall shape when trajectory is overlaid over a point-cloud of object part,
we again utilize Isomap, performing non-linear dimensionality reduction.
% of representing the point-cloud with trajectory.
Prior to performing Isomap, we use the voxel-based cube representation
to jointly represent point-cloud and trajectory %into a common representation space
where each voxel has a count number.
Both the point-cloud and smooth interpolated trajectory is mapped to the corresponding voxel.
%For point-cloud, each point in the point-cloud is mapped to corresponding voxel.
%And for trajectory, each point in the smooth interpolated trajectory
%is mapped to correponding voxel.

\textbf{Language-Trajectory Features} $\phi(l,\tau)$:
%For the feature of language-trajectory $\phi(p,\tau)$, similar to $\phi(p,h)$,
The tensor product of language feature vector
and the trajectory feature is used to capture the relationship between the language and the trajectory:
$\phi(p,\tau) = \phi(p) \otimes \phi(\tau)$.


\subsection{Structured SVM with Latent Variable}

Also as one of our baselines, we used structured SVM with latent variables $\mathcal{H}$
\cite{yu2009learning} using the joint feature map, $\phi(p, l, \tau, h)$,
which consists of additional relations that involve the latent inner joint structure $h$:
$\phi(p,l,\tau,h) = [\phi(\tau); \phi(p,\tau); \phi(l,\tau); \phi(l,h); \phi(p,\tau,h)]$.

%The joint feature of $\phi(p,l,\tau,h)$ is decomposed into a set of different factors to capture
%different relations between point-cloud $p$, language $l$, trajectory $\tau$ and inner joint structure $h$:
%$\phi(p,l,\tau,h) = [\phi(\tau); \phi(p,\tau);\phi(l,\tau); \phi(l,h); \phi(p,\tau,h)]$.



\textbf{Language-Joint Features} $\phi(l,h)$:
%For the feature of language-joint $\phi(p,h)$, 
To capture the relationship between the language and type of joint, which are both discrete, 
we take the tensor product of the language feature vector and the joint type feature vector: 
$\phi(p,h) = \phi(p) \otimes \phi(h)$.
The language feature vector is a bag-of-words in the language,
and the joint type feature vector is a bag of joint types
(i.e. vector of length 3 indicating the existence of each joint type).
The tensor product $\phi(p) \otimes \phi(h)$,
which is a matrix of all possible products between two vectors, 
is reshaped into a vector.









\textbf{PointCloud-Trajectory-Joint Features} $\phi(p,\tau,h)$:
It captures how well point-cloud $p$ and trajectory $\tau$ are
represented by the inner joint structure $h$.
Rather than using whole trajectory, trajectory is broken down into the part 
where it actually interacts with the object $\tau_{inter}$ and the part where it does not $\tau_{no-inter}$.
%Before computing any features, point-cloud is used to separate the trajectory
%into two parts where one is for actual interaction and the rest is for approach of object.

$\phi(p,\tau,h)$ is a concatenation of three types of features, each for a type of joint.
For the ``revolute'' joint, it measures 
the percentage of $\tau_{inter}$ that is within the threshold defined by rotation axis,
the maximum angular rotation occurred while following the threshold,
and the average cosine similarity between the joint rotation axis and the rotation axis computed between trajectory waypoints.
For the ``prismiatic'' joint, it measures
the average cosine similarity between the extension axis and the displacement vector between waypoints.
Finally, for the ``fixed'' joint, it simply checks whether $\tau_{no-inter}$ has collision
with the background since it is important to approach the object from correct angle.
%approaching the object from correct angle is important.








%%%% BELOW NOT USED---------------------------------------------------------------
%%%% BELOW NOT USED---------------------------------------------------------------
%%%% BELOW NOT USED---------------------------------------------------------------
%%%% BELOW NOT USED---------------------------------------------------------------

\iffalse

\subsection{Point Cloud Features}

The point-cloud $p$ needs to be aligned with meaningful coordinate frame.
The center of coordinate is placed at the mean of all points that belong to the part (e.g. ``knob'').
The negative $z$-axis is aligned towards the gravity and the $x$-axis is aligned towards 
the direction of maximum
variance using Principal Component Analysis (PCA) \cite{hsiao2010contact}.

We have implemented following features after the point-cloud of object part has been
axis-aligned:
\begin{itemize}
\item \textbf{Local Shape.}
The local shape is captured by scatterness ($\lambda_0$), linearness ($\lambda_0 - \lambda_1$) 
and planarness ($\lambda_1 - \lambda_2$) \cite{koppula2011semantic}.

\item \textbf{Histogram of Curvature.}
The surface curvature is estimated at each point by the eigenvalues of the covariance matrix,
$\lambda_0 / (\lambda_0 + \lambda_1 + \lambda_2)$ \cite{Rusu_ICRA2011_PCL}.
The curvature at each point is binned into histogram.
\item \textbf{Distribution of Points.}
The bounding box of part is broken down into 3 x 3 x 2 bins and 
the distribution of points is computed.
\item \textbf{Distribution of Nearby Points.}
The points inside $10cm$ radius from the center are again used to compute
distribution of points.
\item \textbf{Ratio of Distribution.}
After computing the distance of farthest point in each dimension,
the ratio between all three dimensions are added as a feature.
\end{itemize}

\fi




\iffalse
With the interpolated smooth trajectory $\tau$, we build following 
histograms by comparing each interpolated point $\tau_i$ in trajectory $\tau$
to previous interpolated points $\tau_j$.
\begin{itemize}
\item \textbf{Histogram of Translation.}
Translation between two points is discretized by direction of translation into
octant as well as amount of displacement.
\item \textbf{Histogram of Rotation Angle.}
Rotation between two points is represented through angle between two quaternions
computed by angle $ = q_2 \cdot q_1^{-1}$.
\item \textbf{Joint Histogram of Translation and Rotation Angle.}
The joint histogram of two features above, translation and rotation angle.
\item \textbf{Histogram of Axis of Rotations.}
Axis of rotation between two points is obtained by calculating the Hamilton product between quaternions of each point, and each axis of rotation is binned into one of 3-d octant.
\end{itemize}
\fi



==> learning.tex <==
% !TEX root = writeup.tex

\subsection{Model Formulation}
We have defined our problem as a structured prediction task of outputting trajectory $\mathcal{T}$
given the point-cloud $\mathcal{P}$ and the language instruction $\mathcal{L}$.
This prediction task has complex and infinitely large output space 
since the trajectories could be of arbitrary length and could follow any arbitrary path.
We use structured support vector machine \cite{tsochantaridis2005large,yu2009learning},
with latent variable $\mathcal{H}$ 
 to learn the discriminant function
$F: \mathcal{P} \times \mathcal{L} \times \mathcal{T} \times \mathcal{H} \rightarrow \mathbb{R}$. 
Learning the discriminant function $F$ results in the following structured support vector machine with latent variable optimization problem:

{
\vskip -.2in
\small
\begin{align*}
\min_{w, \xi}& \frac{1}{2}||w||^2 + C \sum_{i = 1}^{n} \xi_i \qquad  \\
& s.t. \hspace{2.5mm} \forall i: \hspace{2mm} \xi_i \geq 0 \qquad
 \forall i, \hspace{1.5mm} \forall \tau \in \mathcal{T}_o : 
  \max_{h \in \mathcal{H}}  \;\langle w,\phi(p_i, l, \tau_i, h) \rangle 
 - \max_{\hat{h} \in \mathcal{H}} \;\langle w,\phi(p_i, l, \tau, \hat{h}) \rangle 
 \geq \Delta(\tau_i,\tau) - \xi_i 
\end{align*} 
\vskip -.1in
}

%\begin{align*}
%&\min_{w, \xi} \frac{1}{2}||w||^2 + C \sum_{i = 1}^{n} \xi_i \\
%&s.t. \hspace{2.5mm}\forall i: \hspace{2mm} \xi_i \geq 0 \\
%& \hspace{7.5mm} \forall i, \hspace{1.5mm} \forall \tau \in \mathcal{T}_o : 
% \hspace{7.5mm}\max_{h \in \mathcal{H}}  \;\langle w,\phi(p_i, l, \tau_i, h) \rangle 
% - \max_{\hat{h} \in \mathcal{H}} \;\langle w,\phi(p_i, l, \tau, \hat{h}) \rangle 
% \geq \Delta(\tau_i,\tau) - \xi_i 
%\end{align*} 
where $p_i$ is the object part point-cloud and 
$\mathcal{T}_o$ is the set of all trajectories the robot has observed previously
based on our assumption that trajectories could be reused.

\textbf{Latent Variable.}
How an object is operated given its particular shape is due to its internal structure.
%The object is shaped in certain way and is operated in a certain way because of its internal
%structure.
Rather than trying to explicitly learn the articulated structure of the object
\cite{sturm2011probabilistic,burka2013probabilistic},
we treat this internal joint structure as a latent variable $\mathcal{H}$.
Our latent variable $\mathcal{H}$ consists of seven variables 
$(j_t, j_c, j_a) = (j_t, (j_{cx}, j_{cy}, j_{cz}), (j_{ax}, j_{ay}, j_{az}))$
where joint type $j_t \in \{\text{`revolute', `prismatic', `fixed'} \}$.
The center of joint and axis of joint $(j_c, j_a)$ are only used for  `revolute' and `prismatic' joints.
For the `revolute' joint type, $(j_c, j_a)$ represents the center of rotation
and axis of rotation (a unit vector) respectively.
And for `prismatic' joint type, they represent an offset and a unit vector for the direction of extension.
Some definitions of joints are borrowed from \citep{sturm2011probabilistic,burka2013probabilistic}
and Figure~\ref{fig:jointex} shows an example of `revolute' and `prismatic' joints.




\textbf{Learning.}
We used the cutting plane method \cite{yu2009learning} to solve the above optimization problem.
The loss function $\Delta$ and joint feature map $\phi(p,\tau)$ will be 
defined in following Section~\ref{sec:metric} and Section~\ref{sec:features} respectively.
Finding the cutting plane at each iteration involves finding trajectory $\tau$ and the hidden variable $h$
that maximizes: $\max_{\tau, h} \langle w,\phi(p_i, \tau_i,h) \rangle$
and $\max_{\tau, h} \langle w,\phi(p_i, \tau_i,h) \rangle + \Delta(\tau_i,\tau)$.
Our latent variable $h$ is continuous variables except for the type of joint.
We used Limited-memory BFGS \cite{zhu1997algorithm} to find the value of $h$ 
(the joint location and the joint direction).

\textbf{Inference.}
Given the discriminant function $F$, inference step outputs a trajectory $\tau$
that maximizes the discriminant function:
$f(p; \textbf{w}) = \argmax_{\tau \in \mathcal{T}_o} F(p, \tau; \textbf{w})$.
Since the space of trajectory $\mathcal{T}$ can be infinitely large, again based on
our idea that we can transfer trajectories between objects,
we only search through trajectories that it has seen before ($\mathcal{T}_o$) during the training phase.





\iffalse
And we will output a prediction $\textbf{y} \in \mathcal{Y}$ 
(seen during training phase) that maximizes $F$ for a given $\textbf{x} \in \mathcal{X}$:

However, because space of trajectory $Y$ can be infinitely large, we will only
consider trajectory $\textbf{y} \in Y$ that we have seen during training phase.
%similar approach of 
%nearest neighbor to finding best trajectory among the ones we have seen in training phase.
The loss function will be same as evaluation metric that is used to evaluate final result.
And, because our size of training data will limit the search space in $Y$, maximization steps
become feasible.
\fi






